MANDO: Multi-Level Heterogeneous Graph Embeddings for Fine-Grained Detection of Smart Contract Vulnerabilities

Learning heterogeneous graphs consisting of different types of nodes and edges enhances the results of homogeneous graph techniques. An interesting example of such graphs is control-flow graphs representing possible software code execution flows. As such graphs represent more semantic information of code, developing techniques and tools for such graphs can be highly beneficial for detecting vulnerabilities in software for its reliability. However, existing heterogeneous graph techniques are still insufficient in handling complex graphs where the number of different types of nodes and edges is large and variable. This paper concentrates on the Ethereum smart contracts as a sample of software codes represented by heterogeneous contract graphs built upon both control-flow graphs and call graphs containing different types of nodes and links. We propose MANDO, a new heterogeneous graph representation to learn such heterogeneous contract graphs' structures. MANDO extracts customized metapaths, which compose relational connections between different types of nodes and their neighbors. Moreover, it develops a multi-metapath heterogeneous graph attention network to learn multi-level embeddings of different types of nodes and their metapaths in the heterogeneous contract graphs, which can capture the code semantics of smart contracts more accurately and facilitate both fine-grained line-level and coarse-grained contract-level vulnerability detection. Our extensive evaluation of large smart contract datasets shows that MANDO improves the vulnerability detection results of other techniques at the coarse-grained contract level. More importantly, it is the first learning-based approach capable of identifying vulnerabilities at the fine-grained line-level, and significantly improves the traditional code analysis-based vulnerability detection approaches by 11.35% to 70.81% in terms of F1-score.

==> ge-sc-acknowledgment.tex <==
This work was supported by the European Union’s Horizon 2020 research and innovation program under grant agreement No. 833635 (project ROXANNE: Real-time network, text, and speaker analytics for combating organized crime, 2019-2022).


==> ge-sc-material-extended-experiments.tex <==
\subsection{Coarse-Grained Contract-Level Detection with Inputs Being Only Heterogeneous Control-Flow Graphs}
\input{table-cfg-only-coarse-grained-results}
We examine this extended experiment with a similar dataset for each type of bug, presented in Section~\ref{sec:fine-grainedresults} of our main paper. The difference between the two experiments being the input of MANDO is the Heterogeneous Control-Flow Graphs only instead of the Heterogeneous Contract Graphs fused by HCGs and HCFGs. Interestingly, compared the methods achieving the best performance of Table~\ref{tab:f1_cfg} in the main paper to the best ones of Table~\ref{tab:f1_cfg_only_coarse_grained}, we realize that with the inputs from only HCFGs, the Buggy F1 and Macro-F1 of MANDO increase slightly about 1.57\% to 9.17\% with the bugs Time Manipulation and Arithmetic. This problem regards the characteristics of these two vulnerabilities that only depend on the statements inside each function of smart contracts, not the invocation of functions. Therefore, attaching the edge information of HCGs to HCFGs as the fusion form in Heterogenous Contract Graphs may noise the predictions of graph classification tasks. However, MANDO always beat the baseline graph neural networks with a significant gap in detecting smart contracts with bugs, whether inputs of HCFGs-only or the Fused Heterogeneous Contract Graphs.

\subsection{Fine-Grained Function-Level Detection of Smart Contract Vulnerabilities}
In the extended experiment, we propose another fusion form of Heterogeneous Call Graphs and Heterogeneous Control-Flow Graphs, named Form-B Fusion. Different from the core fusion form where the HCFGs are attached to the HCG, each HCFG for a function in the smart contract in Form-B is considered as additional features for the function node in the HCG, and these features are generated by the component ``Topological Graph Neural Network'' in \ourapp, which we describe in Section~\ref{subsec:multi-level-gnn}. Table~\ref{tab:f1_callgraph} shows that our proposed method achieves significant improvements up to 35\% compared to the original metapath2vec method; moreover, it improves F1-score of the predicted bugs slightly by 1\% to 7\% compared to the original node2vec model in all the bug categories.

%Our proposed method could also perform well in detecting smart contract vulnerabilities at the function level. This experiment uses the Heterogeneous Contract Call Graphs as the primary input graphs for the multi-level graph neural networks. Note that each node in a call graph corresponds to a function, and thus that function's control-flow graph. As a fusion with control-flow graphs, each node feature of a heterogeneous call graph fed to the node-level attention heterogeneous GNN is an aggregation of all node embeddings of the corresponding control-flow graph generated by the topological graph neural network. 

\input{table-callgraph-results}



%\input{table-cfg-only-fine-grained-reults}

==> ge-sc-material-gnn.tex <==
We use the four state-of-the-art graph neural networks as baselines in our experiments, including:
\begin{itemize}[leftmargin=1em]
    \item node2vec~\cite{node2vec}: It learns node embeddings by minimizing the cross-entropy loss between the embedding of two nodes belonging to the same random walk with negative sampling.
    \item LINE~\cite{tang2015line}: Generally, LINE only differs from node2vec in the exact formulations of the loss functions and optimizing strategies. It focuses on learning vectors of closer nodes having either connection between them or sharing the same 1-hop neighborhood. Then, the final representation is formed by concatenating the two generated vectors. 
    \item Graph Convolutional Network~\cite{GCN}: The method generalizes the convolutional neural network to solve the node classification problem on graphs. Specifically, it uses the Laplacian matrix as a first-order approximation for the propagation among the layers of spectral graph convolutions.
    \item metapath2vec~\cite{metapath2vec}: For heterogeneous graphs, the embedding of each node will maximize the likelihood of retaining the structures and semantics of the node/edge labels. Similar to node2vec, the negative sampling is obtained during the optimization process.  
    %\item Heterogeneous graph attention network (HAN)~\cite{HAN}: The model includes two level of attention for heterogeneous graph: (i) node level and (ii) semantic level. The former one measures the importance of meta paths of neighbor nodes while the latter one predicts the outcome from the meta paths.
\end{itemize}

==> ge-sc-material-graph-generation.tex <==
The graph extraction tools of Zhuang and Liu et al.~\cite{zhuang2020smart, liu2021smart} have two internal steps. The first step extracts source code from the smart contracts to their pre-defined graph formats. Furthermore, in the second step, they vectorize these graphs to feed their graph neural networks. Notably, each type of bug requires a different tool for extraction and vectorization since it relies on some expert patterns regarding each bug type. This is why their approaches only support two types of vulnerability, including Reentrancy and Time Manipulation, and cannot expand to other bug types. In contrast, the graph generator of the \ourapp framework is an entirely-automatic approach, which does not need any pre-defined patterns. Besides, our generated heterogeneous graphs are sufficiently general to capture the semantic structure of many different vulnerability types: Access Control, Arithmetic, Denial of Service, Front Running, Reentrancy, Time Manipulation, and Unchecked Low-Level Calls. 

We utilize the Smartbugs Wild dataset having 47,398 smart contracts to compare MANDO with their graph extraction tools. In the Reentrancy bug, Zhuang and Liu et al. tools could extract 47279 (99.75\%) contracts but only successfully vectorize 1524 contracts from that and get a total of 3.22\% performance. In the Time Manipulation bug, they could extract 47376 (99.95\%) contracts and also only vectorize 1151 contracts successfully from that and get a total of 2,43\% performance. In the meantime, \ourapp's graph generator and metapath extractor can successfully generate heterogeneous contracts and extract metapaths on 44331/47398 smart contracts for all bug categories before feeding to the multi-level graph neural network, getting 93.53\% in the overall performance.

==> ge-sc-material-vulnerability.tex <==
In this section, we would shortly describe some bug categories collected by Smartbugs or injected by SolidiFI, including:
\begin{itemize}[nosep,leftmargin=1em]
    \item \textit{Access Control}: Failure to use function modifiers or use of tx.origin.
    \item \textit{Arithmetic}: Bugs related to the overflow or underflow of integer.
    \item \textit{Denial of Service}: time-consuming operation leads to the rejection of the smart contract.
    \item \textit{Front Running}: Two dependent transactions that invoke the same contract are included in one block.
    \item \textit{Reentracy}: Unexpected behavior of a contract due to reentrant function calls.
    \item \textit{Time manipulation}: The timestamp of the block is manipulated by the miner.
    \item \textit{Unchecked Low Level Calls}: low level functions i.e. call(), callcode(), delegatecall() or send() fails because of unchecked condition.
\end{itemize}

==> table-callgraph-backup.tex <==
\begin{table*}
\centering
\footnotesize
\label{tab:f1_callgraph}
\label{tab:f1_callgraph}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|} 
\hline
\multicolumn{2}{|c|}{\textbf{Methods }}                                                                                                                                                                                                                                                                               & \multicolumn{1}{c|}{\textbf{Metric}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Access }\\\textbf{Control}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Arithmetic}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Denial of }\\\textbf{Service}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Front }\\\textbf{Running}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Reentrancy}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Time }\\\textbf{Manipulation}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Unchecked Low }\\\textbf{Level Calls}\end{tabular}}  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Original\\Heterogeneous GNN\end{tabular}                                                                                                                                                            & metapath2vec                                                                         & Buggy F1                             & 48.0\%                                                                                          & 62.0\%                                   & 58.0\%                                                                                             & 69.0\%                                                                                         & 49.0\%                                   & 51.0\%                                                                                             & 47.0\%                                                                                                      \\ 
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Original \\Homogeneous GNN\end{tabular}}                                                                                                                                            & GCN                                                                                  & Buggy F1                             & 56\%                                                                                            & 69\%                                     & 64\%                                                                                               & 77\%                                                                                           & 54\%                                     & 61\%                                                                                               & 53\%                                                                                                        \\ 
\cline{2-10}
                                                                                                                                                                                                                               & LINE                                                                                 & Buggy F1                             & 75.0\%                                                                                          & 79.0\%                                   & 79.0\%                                                                                             & 87.0\%                                                                                         & 70.0\%                                   & 74.0\%                                                                                             & 47.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                               & node2vec                                                                             & Buggy F1                             & 81.0\%                                                                                          & 87.0\%                                   & 85.0\%                                                                                             & 89.0\%                                                                                         & 81.0\%                                   & 83.0\%                                                                                             & 77.0\%                                                                                                      \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textit{\textbf{Call Graphs Only.}}\\\textbf{Node-Level Attention}\\\textbf{Heterogeneous GNN with }\\\textbf{Node Features Generated by }\end{tabular}}                              & \begin{tabular}[c]{@{}l@{}}\textbf{NodeType One}\\\textbf{Hot Vectors}\end{tabular}  & Buggy F1                             & 80.0\%                                                                                          & 85.0\%                                   & 83.0\%                                                                                             & \textbf{92.0\% }                                                                               & 78.0\%                                   & 80.0\%                                                                                             & 78.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                               & \textbf{metapath2vec }                                                               & Buggy F1                             & 83.0\%                                                                                          & 80.0\%                                   & 82.0\%                                                                                             & 86.0\%                                                                                         & 79.0\%                                   & 73.0\%                                                                                             & 77.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                               & \textbf{GCN }                                                                        & Buggy F1                             & 72.0\%                                                                                          & 79.0\%                                   & 77.0\%                                                                                             & 87.0\%                                                                                         & 76.0\%                                   & 75.0\%                                                                                             & 72.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                               & \textbf{LINE }                                                                       & Buggy F1                             & 73.0\%                                                                                          & 83.0\%                                   & 76.0\%                                                                                             & 91.0\%                                                                                         & 72.0\%                                   & 71.0\%                                                                                             & 73.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                               & \textbf{node2vec }                                                                   & Buggy F1                             & 72.0\%                                                                                          & 70.0\%                                   & 76.0\%                                                                                             & 89.0\%                                                                                         & 73.0\%                                   & 75.0\%                                                                                             & 71.0\%                                                                                                      \\ 
\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textit{\textbf{Fusion of Call Graphs and}}\\\textit{\textbf{Control-Flow Graphs.}}\\\textbf{Node-Level Attention}\\\textbf{Heterogeneous GNN with }\\\textbf{Node Features Generated by}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\textbf{NodeType One}\\\textbf{Hot Vectors }\end{tabular} & Buggy F1                             & \textbf{83.0\% }                                                                                & 87.0\%                                   & 84.0\%                                                                                             & 86.0\%                                                                                         & 80.0\%                                   & \textbf{85.0\% }                                                                                   & 82.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                               & \textbf{metapath2vec }                                                               & Buggy F1                             & 82.0\%                                                                                          & \textbf{87.0\% }                         & 81.0\%                                                                                             & 89.0\%                                                                                         & 81.0\%                                   & 85.0\%                                                                                             & 77.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                               & \textbf{GCN }                                                                        & Buggy F1                             & 81.0\%                                                                                          & 85.0\%                                   & 82.0\%                                                                                             & 89.0\%                                                                                         & 80.0\%                                   & 84.0\%                                                                                             & 82.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                               & \textbf{LINE }                                                                       & Buggy F1                             & 81.0\%                                                                                          & 86.0\%                                   & 83.0\%                                                                                             & 91.0\%                                                                                         & \textbf{82.0\% }                         & 81.0\%                                                                                             & 80.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                               & \textbf{node2vec }                                                                   & Buggy F1                             & 82.0\%                                                                                          & 87.0\%                                   & 87.0\%                                                                                             & 91.0\%                                                                                         & 80.0\%                                   & 84.0\%                                                                                             & \textbf{84.0\% }                                                                                            \\
\hline
\end{tabular}
\caption{Performance Comparison on Function-Level Search. We use both  \textit{Heterogeneous Contract Call Graphs} and \textit{Heterogeneous Contract Control-Flow Graphs} as the inputs for our Multi-Level Graph Neural Networks. \textit{Buggy F1} means the F1-score of the buggy label.
A total of nine methods are examined in the comparisons. The best performance in each vulnerability category is highlighted.}
\label{tab:f1_callgraph}
\end{table*}

==> table-callgraph-results.tex <==
\begin{table*}
\centering
\footnotesize
\label{tab:f1_callgraph}
\begin{tabular}{|l|l||l||l|l|l|l|l|l|l|} 
\hline
\multicolumn{2}{|c||}{\begin{tabular}[c]{@{}c@{}}\\\textbf{Methods }\end{tabular}}                                                                                                                                                                                                                                   & \multicolumn{1}{c||}{\textbf{Metric}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Access }\\\textbf{Control}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Arithmetic}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Denial of }\\\textbf{Service}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Front }\\\textbf{Running}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Reentrancy}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Time }\\\textbf{Manipulation}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Unchecked Low }\\\textbf{Level Calls}\end{tabular}}  \\ 
\hhline{|==::=::=======|}
\begin{tabular}[c]{@{}l@{}}Original\\Heterogeneous GNN\end{tabular}                                                                                                                                                           & metapath2vec                                                                         & Buggy F1                              & 48.0\%                                                                                          & 62.0\%                                   & 58.0\%                                                                                             & 69.0\%                                                                                         & 49.0\%                                   & 51.0\%                                                                                             & 47.0\%                                                                                                      \\ 
\hhline{|==::=::=======|}
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Original \\Homogeneous GNN\end{tabular}}                                                                                                                                           & GCN                                                                                  & Buggy F1                              & 56\%                                                                                            & 69\%                                     & 64\%                                                                                               & 77\%                                                                                           & 54\%                                     & 61\%                                                                                               & 53\%                                                                                                        \\ 
\cline{2-10}
                                                                                                                                                                                                                              & LINE                                                                                 & Buggy F1                              & 75.0\%                                                                                          & 79.0\%                                   & 79.0\%                                                                                             & 87.0\%                                                                                         & 70.0\%                                   & 74.0\%                                                                                             & 47.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                              & node2vec                                                                             & Buggy F1                              & 81.0\%                                                                                          & 87.0\%                                   & 85.0\%                                                                                             & 89.0\%                                                                                         & 81.0\%                                   & 83.0\%                                                                                             & 77.0\%                                                                                                      \\ 
\hhline{|==::=::=======|}
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textit{\textbf{Fusion (Form-B) of}}\\\textit{\textbf{Call Graphs and}}\\\textit{\textbf{Control-Flow Graphs.}}\\\textbf{\ourapp with Node}\\\textbf{Features Generated by}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\textbf{NodeType One}\\\textbf{Hot Vectors }\end{tabular} & Buggy F1                              & \textbf{83.0\% }                                                                                & 87.0\%                                   & 84.0\%                                                                                             & 86.0\%                                                                                         & 80.0\%                                   & \textbf{85.0\% }                                                                                   & 82.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                              & \textbf{metapath2vec }                                                               & Buggy F1                              & 82.0\%                                                                                          & \textbf{87.0\% }                         & 81.0\%                                                                                             & 89.0\%                                                                                         & 81.0\%                                   & 85.0\%                                                                                             & 77.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                              & \textbf{GCN }                                                                        & Buggy F1                              & 81.0\%                                                                                          & 85.0\%                                   & 82.0\%                                                                                             & 89.0\%                                                                                         & 80.0\%                                   & 84.0\%                                                                                             & 82.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                              & \textbf{LINE }                                                                       & Buggy F1                              & 81.0\%                                                                                          & 86.0\%                                   & 83.0\%                                                                                             & \textbf{91.0\% }                                                                               & \textbf{82.0\% }                         & 81.0\%                                                                                             & 80.0\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                                                                              & \textbf{node2vec }                                                                   & Buggy F1                              & 82.0\%                                                                                          & 87.0\%                                   & \textbf{87.0\% }                                                                                   & 91.0\%                                                                                         & 80.0\%                                   & 84.0\%                                                                                             & \textbf{84.0\% }                                                                                            \\
\hline
\end{tabular}
% \lxnote{May replace some methods' name with our approach's shortname \ourapp.}
\caption{\small Performance Comparison on the Fine-Grained Function-Level Detection. We use \textit{Heterogeneous Call Graphs} of the Buggy Smart Contracts as the inputs for \ourapp framework, with \textit{Heterogeneous Control-Flow Graphs} as the additional features of the function nodes of the input graphs. \textit{Buggy F1} means the F1-score of the buggy function-node label. The best performance in each vulnerability category is highlighted.}
\label{tab:f1_callgraph}
\end{table*}

==> table-cfg-backup.tex <==
\begin{table*}
\centering
\footnotesize
\begin{tabular}{|l|l||l||l|l|l|l|l|l|l|} 
\hline
\multicolumn{2}{|c||}{\textbf{Methods }}                                                                                                                                                                                                                                            & \multicolumn{1}{c||}{\textbf{Metrics}}                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Access }\\\textbf{Control}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Arithmetic}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Denial of }\\\textbf{Service}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Front }\\\textbf{Running}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Reentrancy}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Time }\\\textbf{Manipulation}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Unchecked Low }\\\textbf{Level Calls}\end{tabular}}  \\ 
\hline \hline
\multirow{12}{*}{\begin{tabular}[c]{@{}l@{}}Conventional \\Detection Tools\end{tabular}}                                                                                    & \multirow{2}{*}{securify}                                                                            & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 13.0\%                                                                                          & 0.0\%                                    & 18.0\%                                                                                             & 53.0\%                                                                                         & 23.0\%                                   & 24.0\%                                                                                             & 11.0\%                                                                                                      \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 52.3\%                                                                                          & 45.2\%                                   & 52.0\%                                                                                             & 72.2\%                                                                                         & 58.4\%                                   & 52.4\%                                                                                             & 54.1\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{mythril}                                                                             & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 34.0\%                                                                                          & 73.0\%                                   & 41.0\%                                                                                             & 63.0\%                                                                                         & 19.0\%                                   & 23.0\%                                                                                             & 14.0\%                                                                                                      \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 61.1\%                                                                                          & \textbf{84.1\%}                          & 60.1\%                                                                                             & 77.8\%                                                                                         & 55.3\%                                   & 50.8\%                                                                                             & 55.7\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{slither}                                                                             & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 32.0\%                                                                                          & 0.0\%                                    & 13.0\%                                                                                             & 26.0\%                                                                                         & 15.0\%                                   & 44.0\%                                                                                             & 10.0\%                                                                                                      \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 61.5\%                                                                                          & 45.2\%                                   & 42.7\%                                                                                             & 56.9\%                                                                                         & 49.4\%                                   & 57.3\%                                                                                             & 53.3\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{manticore}                                                                           & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 30.0\%                                                                                          & 30.0\%                                   & 12.0\%                                                                                             & 7.0\%                                                                                          & 9.0\%                                    & 24.0\%                                                                                             & 4.0\%                                                                                                       \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 61.1\%                                                                                          & 61.0\%                                   & 48.0\%                                                                                             & 46.9\%                                                                                         & 51.2\%                                   & 55.1\%                                                                                             & 50.6\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{smartcheck}                                                                          & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 20.0\%                                                                                          & 22.0\%                                   & 52.0\%                                                                                             & 0.0\%                                                                                          & 22.0\%                                   & 44.0\%                                                                                             & 11.0\%                                                                                                      \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 56.0\%                                                                                          & 56.1\%                                   & 69.9\%                                                                                             & 46.2\%                                                                                         & 57.8\%                                   & 64.2\%                                                                                             & 54.1\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{oyente}                                                                              & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 21.0\%                                                                                          & 71.0\%                                   & 48.0\%                                                                                             & 0.0\%                                                                                          & 20.0\%                                   & 24.0\%                                                                                             & 8.0\%                                                                                                       \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 57.3\%                                                                                          & 82.8\%                                   & 67.2\%                                                                                             & 44.8\%                                                                                         & 56.1\%                                   & 52.4\%                                                                                             & 52.6\%                                                                                                      \\ 
\hline \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Original\\Heterogeneous GNN\end{tabular}}                                                                       & \multirow{2}{*}{metapath2vec}                                                                        & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 28.0\%                                                                                                & 59.0\%                                         & 61.0\%                                                                                                & 80.0\%                                                                                               & 58.0\%                                         & 57.0\%                                                                                                   & 16.0\%                                                                                                            \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 46.31\%                                                                                                & 48.45\%                                         & 44.67\%                                                                                                   & 45.68\%                                                                                               & 50.22\%                                         & 49.73\%                                                                                                   & 48.48\%                                                                                                            \\ 
\hline \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Original \\Homogeneous GNNs\end{tabular}}                                                                        & \multirow{2}{*}{GCN}                                                                                 & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 50.0\%                                                                                          & 69.0\%                                   & 61.0\%                                                                                             & 79.0\%                                                                                         & 58.0\%                                   & 65.0\%                                                                                             & 14.0\%                                                                                                      \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 52.8\%                                                                                          & 45.8\%                                   & 50.7\%                                                                                             & 49.9\%                                                                                         & 51.7\%                                   & 52.2\%                                                                                             & 46.5\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{LINE}                                                                                & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 20.0\%                                                                                          & 65.0\%                                   & 59.0\%                                                                            & 81.0\%                                                                                         & 74.0\%                                   & 69.0\%                                                                                             & 1.0\%                                                                                                       \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 43.6\%                                                                                          & 47.3\%                                   & 51.1\%                                                                                             & 45.1\%                                                                                         & 37.1\%                                   & 50.2\%                                                                                             & 41.3\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{node2vec}                                                                            & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 43.0\%                                                                                          & 69.0\%  & 62.0\%                                                                                             & 83.0\%                                                                                         & 76.0\%                                   & 69.0\%                                                                                             & 4.0\%                                                                                                       \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 55.5\%                                                                                          & 57.2\%                                   & 54.8\%                                                                                             & 46.7\%                                                                                         & 60.5\%                                   & 53.5\%                                                                                             & 42.3\%                                                                                                      \\ 
\hline \hline
\multirow{10}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Node-Level Attention }\\\textbf{Heterogeneous GNN }\\\textbf{with Node Features }\\\textbf{Generated by }\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{NodeType One}\\\textbf{Hot Vectors}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 74.0\%                                                                                          & 76.0\%                                   & 70.0\%                                                                                             & 86.0\%                                                                                         & 80.0\%                                   & 81.0\%                                                                                             & 3.0\%                                                                                                       \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 70.2\%                                                                                          & 67.7\%                                   & 63.6\%                                                                                             & 62.5\%                                                                                         & 60.5\%                                   & 77.0\%                                                                                             & 41.8\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{\textbf{metapath2vec }}                                                              & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 59.0\%                                                                                          & 66.0\%                                   & 66.0\%                                                                                             & 83.0\%                                                                                         & 68.0\%                                   & 68.0\%                                                                                             & 24.0\%                                                                                                      \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 61.8\%                                                                                          & 60.0\%                                   & 55.3\%                                                                                             & 62.7\%                                                                                         & 61.2\%                                   & 67.8\%                                                                                             & 49.1\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{\textbf{GCN }}                                                                       & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 62.0\%                                                                                          & 73.0\%                                   & 65.0\%                                                                                             & 85.0\%                                                                                         & 68.0\%                                   & 72.0\%                                                                                             & 19.0\%                                                                                                      \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 60.0\%                                                                                          & 61.9\%                                   & 62.1\%                                                                                             & 59.3\%                                                                                         & 60.1\%                                   & 70.7\%                                                                                             & 47.3\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{\textbf{LINE }}                                                                      & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & \textbf{78.0\%}                                                                                 & 80.0\%                                   & \textbf{77.0\%}                                                                                    & 87.0\%                                                                                         & \textbf{82.0\%}                          & 88.0\%                                                                                             & 79.0\%                                                                                                      \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & \textbf{76.2\%}                                                                                 & 73.3\%                                   & \textbf{72.8\%}                                                                                    & \textbf{75.6\%}                                                                                & \textbf{76.8\%}                          & \textbf{83.6\%}                                                                                    & 80.9\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{\textbf{node2vec }}                                                                  & \begin{tabular}[c]{@{}l@{}}Buggy Label\\F1-score\end{tabular} & 78.0\%                                                                                          & \textbf{82.0\%}                          & 77.0\%                                                                                             & \textbf{88.0\%}                                                                                & 81.0\%                                   & \textbf{89.0\%}                                                                                    & \textbf{82.0\%}                                                                                             \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Overall\\Macro-F1\end{tabular}     & 73.1\%                                                                                          & 73.4\%                                   & 70.0\%                                                                                             & 71.5\%                                                                                         & 76.5\%                                   & 83.0\%                                                                                             & \textbf{82.9\%}                                                                                             \\
\hline
\end{tabular}
\caption{Performance comparison. We use the  Heterogeneous Contract Control-Flow Graphs as the inputs for our Multi-Level Graph Neural Networks. A total of fifteen methods are examined in the comparisons. The best performance in each bug type is highlighted.}
\label{tab:f1_cfg}
\end{table*}

==> table-cfg-only-coarse-grained-results.tex <==
%!TeX root=ge-sc-main.tex

\begin{table*}
\centering
\footnotesize
\begin{tabular}{|l|l||l||l|l|l|l|l|l|l|} 
\hline
\multicolumn{2}{|c||}{\textbf{Methods }}                                                                                                                                                                                                                                            & \multicolumn{1}{c||}{\textbf{Metrics}}                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Access }\\\textbf{Control}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Arithmetic}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Denial of }\\\textbf{Service}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Front }\\\textbf{Running}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Reentrancy}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Time }\\\textbf{Manipulation}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Unchecked Low }\\\textbf{Level Calls}\end{tabular}}  \\

\hline \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Original\\Heterogeneous GNN\end{tabular}} 
& \multirow{2}{*}{metapath2vec}  
& \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 38.40\%	& 47.36\%	& 39.93\%	& 26.84\%	& 32.84\%	& 32.68\%	& 41.63\%  \\
\cline{3-10}  &  & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}
& 41.11\%	& 44.73\%	& 38.27\%	& 33.46\%	& 43.02\%	& 40.98\%	& 43.49\%  \\
\hline \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Original \\Homogeneous GNNs\end{tabular}}           & \multirow{2}{*}{GCN}                                                                         & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 39.98\%	& - 	& 45.25\%	& - 	& -  	& 36.66\%	& -    \\ 
\cline{3-10} & & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}  
& 38.87\%	& - 	& 37.79\%	& -  	& -  	& 41.91\%	& -    \\ 
\cline{2-10} & \multirow{2}{*}{LINE} & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 39.10\%	& 42.20\%	& 51.21\%	& 42.14\%	& 53.00\%	& 43.45\%	& 52.26\%  \\
\cline{3-10} & & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}     
& 33.43\%	& 33.12\%	& 32.18\%	& 29.11\%	& 36.59\%	& 33.09\%	& 33.91\%  \\
\cline{2-10} & \multirow{2}{*}{node2vec}                                                        & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 39.56\%	& 43.67\%	& 53.43\%	& 47.84\%	& 57.04\%	& 45.62\%	& 50.21\%  \\
\cline{3-10} &    & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular} 
& 38.52\%	& 37.33\%	& 39.77\%	& 35.73\%	& 44.08\%	& 37.24\%	& 46.58\%  \\


\hline \hline
\multirow{10}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\textit{HCFGs only.}}\\\textbf{\ourapp with}\\\textbf{Node Features }\\\textbf{Generated by }\end{tabular}} & \multirow{2}{*}{
\begin{tabular}[c]{@{}l@{}}\textbf{NodeType One}\\\textbf{Hot Vectors}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& \textbf{69.99\%}	& \textbf{76.04\%}	& 83.85\%	& 84.04\%	& \textbf{70.20\%}	& \textbf{89.35\%}	& \textbf{69.61\%}	\\
\cline{3-10}  &  & \begin{tabular}[c]{@{}l@{}}Macro-F1 \end{tabular}
& \textbf{69.23\%}	& \textbf{77.24\%}	& 82.67\%	& 80.37\%	& \textbf{72.91\%}	& \textbf{88.48\%}	& \textbf{70.86\%}	\\
\cline{2-10} & \multirow{2}{*}{\textbf{metapath2vec }}
& \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular}
& 53.99\%	& 53.94\%	& 59.14\%	& 61.34\%	& 52.26\%	& 56.55\%	& 49.69\%	\\
\cline{3-10} &   & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}
& 55.97\%	& 56.82\%	& 61.12\%	& 64.54\%	& 58.53\%	& 58.65\%	& 54.75\%	\\
\cline{2-10} & \multirow{2}{*}{\textbf{GCN }}
& \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 45.31\%	& -    & 55.71\%	& -	& -	& 50.17\%   & -	\\
\cline{3-10} & & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular} 
& 49.10\%	& -    & 63.41\%	& -	& -	& 58.09\%   & - \\
\cline{2-10} & \multirow{2}{*}{\textbf{LINE }} 
& \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 64.10\%	& 60.46\%	& \textbf{85.22\%}	& \textbf{87.23\%}	& 44.40\%	& 87.54\%	& 54.84\%	\\
\cline{3-10} &  & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular} 
& 66.47\%	& 67.65\%	& \textbf{84.36\%}	& \textbf{84.37\%}	& 58.83\%	& 87.80\%	& 62.73\%	\\
\cline{2-10} & \multirow{2}{*}{\textbf{node2vec }} & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 59.55\%	& 60.42\%	& 81.50\%	& 83.77\%	& 56.69\%	& 75.29\%	& 56.17\%	\\
\cline{3-10} &  & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}
& 66.96\%	& 67.55\%	& 80.03\%	& 80.01\%	& 66.47\%	& 76.44\%	& 64.32\%	\\

\hline
\end{tabular}
 %\lxnote{May replace some methods' name with our approach's shortname \ourapp.}
\caption{\small Performance Comparison on the Coarse-Grained Contract-Level Detection. We use the \textit{Heterogeneous Control-Flow Graphs} of both Clean and Buggy Smart Contracts as the inputs for \ourapp framework. \textit{Buggy- F1} means the F1-score of the buggy graph label. The best performance in each vulnerability category is highlighted. ‘–’ denotes not applicable due to the insufficiency of GPU memory to handle the input graphs for GCN model.}
\label{tab:f1_cfg_only_coarse_grained}
\end{table*}

==> table-cfg-only-fine-grained-reults.tex <==
%!TeX root=ge-sc-main.tex

\begin{table*}
\centering
\footnotesize
\begin{tabular}{|l|l||l||l|l|l|l|l|l|l|} 
\hline
\multicolumn{2}{|c||}{\textbf{Methods }}                                                                                                                                                                                                                                            & \multicolumn{1}{c||}{\textbf{Metrics}}                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Access }\\\textbf{Control}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Arithmetic}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Denial of }\\\textbf{Service}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Front }\\\textbf{Running}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Reentrancy}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Time }\\\textbf{Manipulation}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Unchecked Low }\\\textbf{Level Calls}\end{tabular}}  \\ 
\hline \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Original\\Heterogeneous GNN\end{tabular}}                                                                       & \multirow{2}{*}{metapath2vec}                                                                        & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} & 28.0\%                                                                                                & 59.0\%                                         & 61.0\%                                                                                                & 80.0\%                                                                                               & 58.0\%                                         & 57.0\%                                                                                                   & 16.0\%                                                                                                            \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}     & 46.3\%                                                                                                & 48.5\%                                         & 44.7\%                                                                                                   & 45.7\%                                                                                               & 50.2\%                                         & 49.7\%                                                                                                   & 48.5\%                                                                                                            \\ 
\hline \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Original \\Homogeneous GNNs\end{tabular}}                                                                        & \multirow{2}{*}{GCN}                                                                                 & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} & 50.0\%                                                                                          & 69.0\%                                   & 61.0\%                                                                                             & 79.0\%                                                                                         & 58.0\%                                   & 65.0\%                                                                                             & 14.0\%                                                                                                      \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}     & 52.8\%                                                                                          & 45.8\%                                   & 50.7\%                                                                                             & 49.9\%                                                                                         & 51.7\%                                   & 52.2\%                                                                                             & 46.5\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{LINE}                                                                                & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} & 20.0\%                                                                                          & 65.0\%                                   & 59.0\%                                                                            & 81.0\%                                                                                         & 74.0\%                                   & 69.0\%                                                                                             & 1.0\%                                                                                                       \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}     & 43.6\%                                                                                          & 47.3\%                                   & 51.1\%                                                                                             & 45.1\%                                                                                         & 37.1\%                                   & 50.2\%                                                                                             & 41.3\%                                                                                                      \\ 
\cline{2-10}
                                                                                                                                                                            & \multirow{2}{*}{node2vec}                                                                            & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} & 43.0\%                                                                                          & 69.0\%  & 62.0\%                                                                                             & 83.0\%                                                                                         & 76.0\%                                   & 69.0\%                                                                                             & 4.0\%                                                                                                       \\ 
\cline{3-10}
                                                                                                                                                                            &                                                                                                      & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}     & 55.5\%                                                                                          & 57.2\%                                   & 54.8\%                                                                                             & 46.7\%                                                                                         & 60.5\%                                   & 53.5\%                                                                                             & 42.3\%                                                                                                      \\ 
\hline \hline
\multirow{12}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{\textit{CFGs only.}}\\\textbf{\ourapp with}\\\textbf{Node Features }\\\textbf{Generated by }\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{NodeType One}\\\textbf{Hot Vectors}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 71.97\%	& 77.90\%	& 75.18\%	& 85.46\%	& 79.76\%	& 81.01\%	& 23.53\% \\
\cline{3-10}  &  & \begin{tabular}[c]{@{}l@{}}Macro-F1 \end{tabular}
& 68.63\%	& 70.35\%	& 69.32\%	& 60.22\%	& 70.20\%	& 77.52\%	& 51.93\% \\
\cline{2-10} & \multirow{2}{*}{\textbf{metapath2vec }}
& \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 55.89\%	& 67.42\%	& 58.51\%	& 83.15\%	& 70.32\%	& 68.50\%	& 25.95\% \\ 
\cline{3-10} &   & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}
& 60.85\%	& 61.38\%	& 58.52\%	& 59.70\%	& 63.11\%	& 68.09\%	& 52.42\% \\
\cline{2-10} & \multirow{2}{*}{\textbf{GCN }}
& \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 58.98\%	& 70.00\%	& 62.72\%	& 84.91\%	& 71.06\%	& 71.86\%	& 27.48\% \\
\cline{3-10} & & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular} 
& 61.43\%	& 63.22\%	& 60.10\%	& 58.76\%	& 63.01\%	& 71.08\%	& 53.04\% \\ 
\cline{2-10} & \multirow{2}{*}{\textbf{LINE }} 
& \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& 76.71\%	& 79.06\%	& \textbf{78.28\%}	& \textbf{88.24\%}	& 82.67\%	& 85.47\%	& 73.70\% \\
\cline{3-10} &  & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular} 
& \textbf{75.08\%}	& 73.70\%	& \textbf{73.33\%}	& 71.52\%	& 75.23\%	& 81.56\%	& 77.94\% \\
\cline{2-10} & \multirow{2}{*}{\textbf{node2vec }} & \begin{tabular}[c]{@{}l@{}}Buggy F1\end{tabular} 
& \textbf{76.98\%}	& \textbf{81.65\%}	& 78.15\%	& 88.23\%	& \textbf{83.03\%}	& \textbf{86.37\%}	& \textbf{74.37\%} \\ 
\cline{3-10} &  & \begin{tabular}[c]{@{}l@{}}Macro-F1\end{tabular}
& 72.73\%	& 74.98\%	& 71.73\%	& \textbf{71.65\%}	& \textbf{77.13\%}	& \textbf{81.69\%}	& \textbf{78.68\%} \\ 

\hline
\end{tabular}
 %\lxnote{May replace some methods' name with our approach's shortname \ourapp.}
\caption{CFG only of Fine-Grained Tasks}
\label{tab:f1_cfg_only_fine_grained}
\end{table*}

==> tikz-flowchart.tex <==
% \documentclass[border=3mm,
%                tikz]{standalone}
%\usetikzlibrary{arrows.meta,
%                calc, chains,
%                quotes,
%                positioning,
%                shapes.geometric}

%\begin{document}

\resizebox{0.33\textwidth}{!}{%
 \begin{tikzpicture}[ 
    node distance = 8mm and 16mm,
      start chain = A going below,
      base/.style = {draw, minimum width=32mm, minimum height=8mm,
                     align=center, on chain=A},
 normal/.style = {base, rectangle, rounded corners},
 collored/.style = {base, rectangle, rounded corners, fill=yellow!30},
  every edge quotes/.style = {auto=right}]
                    
\node [normal]       {reentrancy\_simple.sol\_Reentrance\_withdrawBalance()};      % <-- A-1
\node [normal]         {Node Type: ENTRY\_POINT};
\node [collored]              {Node Type: IF\\EXPRESSION:\\!(msg.sender.call.value(userBalance[msg.sender])())};
\node [normal]         {Node Type: THROW};
\node [normal, right=of A-4]        {Node Type: END\_IF};
\node [normal]         {Node Type: EXPRESSION\\EXPRESSION:\\userBalance[msg.sender]=0};        % <-- A-6
%%
\draw [arrows=-Stealth] 
    (A-1) edge["Next"]          (A-2)
    (A-2) edge["Next"]    (A-3)
    (A-3) edge["True"]       (A-4)
    (A-3) edge["False"]            (A-5)
    (A-5) edge["Next"]          (A-6)
    ;
  \end{tikzpicture}
 } 
% \end{document}
